SonicRAG : High Fidelity Sound Effects Synthesis Based on Retrival Augmented Generation

Large Language Models (LLMs) have demonstrated remarkable capabilities in natural language processing (NLP) and multimodal learning, with successful applications in text generation and speech synthesis, enabling a deeper understanding and generation of multimodal content. In the field of sound effects (SFX) generation, LLMs have been leveraged to orchestrate multiple models for audio synthesis. However, due to the scarcity of annotated datasets, and the complexity of temproal modeling. current SFX generation techniques still fall short in achieving high-fidelity audio. To address these limitations, this paper introduces a novel framework that integrates LLMs with existing sound effect databases, allowing for the retrieval, recombination, and synthesis of audio based on user requirements. By leveraging this approach, we enhance the diversity and quality of generated sound effects while eliminating the need for additional recording costs, offering a flexible and efficient solution for sound design and application.

==> Sections/featrues.tex <==
%\subsection{Analysis}
%Sound design plays a crucial role in multimedia industries such as film and game design. Well-crafted sound effects enhance immersion, elevating the overall experience. For sound designers who have already built extensive sound libraries, the key challenge is efficiently analyzing creative intent and transforming imagination into high-quality sound effects.
%
%SonicRAG addresses this need by facilitating an interactive dialogue, iteratively refining the designer’s vision and seamlessly blending existing assets into a cohesive result. The following demonstrates SonicRAG in real-world applications:
%
%\begin{figure}[!ht]
%	\centering
%	\includegraphics[width=1\textwidth]{Figures/behavior.pdf}
%	\caption{Behavior of SonicRAG in diffrent working situation. Left side shows how is RAG and Mixer enable LLM to synthsis audio. another depicts adjustability of framework. Right part exhibits multimodel LLM can understand onomatopoeias and represent it to other media.}
%	\label{fig:behavior}
%\end{figure} 

%\subsection{Comparision}
%SonicRAG can reuse pre-recorded sound assets and synthesize sound effects through Mixer Script, giving it an advantage in both sound quality and precise sound adjustment. Additionally, by leveraging multimodal training, LLMs can be further extended to achieve speech-to-sound and even onomatopoeia-to-sound generation. See Table \ref{tab:comparison} compares SonicRAG with existing.
%
%\begin{table}[h]
%	\centering
%	\renewcommand{\arraystretch}{1.3} 
%	\setlength{\tabcolsep}{10pt} 
%	\begin{tabular}{lccc} 
%		\toprule
%		Method & Native sampling & Precise editing by text & onomatopoeia to sound\\
%		\midrule
%		AudioLDM & \xmark & \xmark & \xmark \\
%		AudioGen  &\xmark & \xmark & \xmark  \\
%		WavCraft  &\xmark & \cxmark & \cxmark \\
%		WavJourney  &\xmark & \cxmark & \cxmark \\
%		SonicRAG  &\cmark & \cmark & \cmark \\
%		\bottomrule
%	\end{tabular}
%	\caption{\emph{Comparison of capabilities between SonicRAG and recent audio generation methods, Due to the limitations of neural network models, previous approaches had to downsample the signal to around 16kHz or use spectrogram-based training and generation.While this yields satisfactory results for speech synthesis, the loss of details caused by aliasing becomes more apparent in sound effects. Precise editing means user could adjust components detail(e.g. Frequency, Dynamics and Voice onset time) of sound. Audio generation based on Latent Diffusion Models is difficult to control, even though LLMs can understand onomatopoeia and abstract concepts, they still cannot reliably produce the desired results on WavCraft and WavJourney.}}
%	\label{tab:comparison}
%\end{table}


==> Sections/limit.tex <==
\subsection{Limitation}
SonicRAG provide user an creative and interactive interface for synthesis high fidelity sound effect. But it still have limitations: 1): Infrastructure: the framework needs user already have text-relational audio files for assets. 2): Perception: Due to different sense of hearing, capability of effects provided by Mixer Script may not enough for everyone. 3): Efficiency: it require larger size LLMs such as GPT-4o for comprehend abstract tasks. 
\subsection{Future Work}
Use sounds to assemble anothers is a complex problem that encompasses multiple disciplines like SEC(sound event classfication), SED(sound event detection with timestamp) and ASC(Acoustic sence classification). It isn't solved effectively in textual-based methods so far. Future research could explore using task-specific pre-trained embeddings to assist in fine-tuning LLMs, optimizing their performance for sound synthesis.

